The Tensor Data Platform: Towards an AI-centric Database System

Database engines have historically absorbed many of the innovations in data processing, adding features to process graph data, XML, object oriented, and text among many others. In this paper, we make the case that it is time to do the same for AI -- but with a twist! While existing approaches have tried to achieve this by integrating databases with external ML tools, in this paper we claim that achieving a truly AI-centric database requires moving the DBMS engine, at its core, from a relational to a tensor abstraction. This allows us to: (1) support multi-modal data processing such as images, videos, audio, text as well as relational; (2) leverage the wellspring of innovation in HW and runtimes for tensor computation; and (3) exploit automatic differentiation to enable a novel class of "trainable" queries that can learn to perform a task. To support the above scenarios, we introduce TDP: a system that builds upon our prior work mapping relational queries to tensors. Thanks to a tighter integration with the tensor runtime, TDP is able to provide a broader coverage of new emerging scenarios requiring access to multi-modal data and automatic differentiation.

==> limitations.tex <==
\section{Challenges and Opportunities}

We believe that having an AI-centric database will open several possibilities that are currently out of reach to traditional database systems. We shave shown some of these examples in Section~\ref{sec:use-cases}.
Nevertheless, we see several challenges ahead of us, and hopefully many opportunities. We list few of these next.

\stitle{Limits of SQL as declarative ML tool.}
The biggest open question for us right now is to which extent SQL can be used to declaratively express ML tasks. We already described how LLP problems can be mapped into group by-count aggregate queries, but does this apply to other classes of SQL queries? We are currently investigating this question and indeed we are finding interesting parallels between classes of SQL and ML tasks. For instance, queries with order by clauses can be mapped to learning to rank~\cite{learning-to-rank} tasks once we add differentiable sorting~\cite{differentiable-sorting} support in \system. Similarly, we could change the query of Section~\ref{sec:query-on-images} to sum numbers extracted from the images. This task is closer to neurosymbolic systems such as scallops~\cite{scallop}.

\stitle{Indexing.}
\system currently does not support exact (e.g., regular database indexes) nor approximate indexes (e.g., approximate-nearest-neighbor-based indexes such as the one used in vector search databases~\cite{milvus,analyticdb-v}).
Integrating approximate indexing in \system shouldn't be too hard, and since approximate index search is used in conjunction with top-k queries %(Top-k can be implemented in SQL using order-by and limit statements% and
a top-k query triggering lookups into an approximate index can be probably expressed in SQL using a mix between order-by, limit and  UDFs used to define as domain of the order by clause.
Regarding exact indexes, an open question we have is whether we can learn indexes~\cite{learned-index} together with the query, so that we can optimize both for the ML task and data access.

\stitle{ETL, Encodings and Materialized Views.}
One interesting aspect about \system is that it can store both row data (e.g., images) as well as encodings and embeddings.
From this point of view, we can build several layers of encodings and ML-generated embeddings defining different semantics layers on top of raw data. This is similar to ETL processes in data warehousing settings, but it can be executed within a unified system.

\stitle{Scalability.}
One major open challenge we foresee is scaling the database system.
Unstructured data such images and video require a lot of space, and distributed processing is assuredly needed.
While tensor runtimes already provide primitives for distributed processing, these are based on the MPI abstraction which does not naturally map to how queries are often executed in distributed settings (e.g., using shuffle/exchange operators).
On top of this, being able to appropriately balance computations across multiple CPUs, GPUs, or other hardware accelerators is a hard and really important task if we want to maximize the utilization of the available resources.


% \mi{Matteo, Apurva}
% \begin{itemize}
% \item SQL top k can (if aprox) be mapped into Miluvs like systems.
%     \item Can we learn data access together with the query? I.e., can we merge learning the task with learning how do it efficiently?
%     \item What are the limits of using SQL to learn a task?
%     \item What are the limits of the tensor abstraction? For instance operator fusion is really hard over tensors with undefined output shapes (e.g., filters).
%     \item What is the proper storage format for tensor data, which allow both efficient retrieving and fast updates? Tensor are mostly threaten as in memory-format in fact AFAIK.
%     \item multiple encodings as views over raw data.
% \end{itemize}
